Only Time Can Tell: Discovering Temporal Data for Temporal Modeling

Understanding temporal information and how the visual world changes over time is a fundamental ability of intelligent systems. In video understanding, temporal information is at the core of many current challenges, including compression, efficient inference, motion estimation or summarization. However, in current video datasets it has been observed that action classes can often be recognized without any temporal information from a single frame of video. As a result, both benchmarking and training in these datasets may give an unintentional advantage to models with strong image understanding capabilities, as opposed to those with strong temporal understanding. In this paper we address this problem head on by identifying action classes where temporal information is actually necessary to recognize them and call these "temporal classes". Selecting temporal classes using a computational method would bias the process. Instead, we propose a methodology based on a simple and effective human annotation experiment. We remove just the temporal information by shuffling frames in time and measure if the action can still be recognized. Classes that cannot be recognized when frames are not in order are included in the temporal Dataset. We observe that this set is statistically different from other static classes, and that performance in it correlates with a network's ability to capture temporal information. Thus we use it as a benchmark on current popular networks, which reveals a series of interesting facts. We also explore the effect of training on the temporal dataset, and observe that this leads to better generalization in unseen classes, demonstrating the need for more temporal data. We hope that the proposed dataset of temporal categories will help guide future research in temporal modeling for better video understanding.

==> figures/human_vs_machine.tex <==
\subsection{Humans vs Machines}
% python notebook: plot acc and regression 
% python notebook: Plot Correlation by Group and Class (all datasets) 
%\lt{You may want to explain why you are presenting this analysis. It is introduced without context.}
Since our selection process is based on human perception, one may wonder if the recognition complexity of action classes similar for humans and machines. In other words, if a class is more ambiguous or harder for humans, is it also ambiguous or hard to identify for modern networks? We take the R(2+1)D model and measure correlation of per-class accuracy {\em without temporal shuffling} between humans and machines. %Results are shown in Fig.~\ref{fig:human_vs_machine_r3d}, 
We observe a positive correlation (Pearson correlation coefficient is 0.22) with high confidence (p-value is 0.001). Classes that are more ambiguous or harder for humans are also so for machines. For example both humans and machines find it hard to recognize  ``interviewing with camera" (confused with ``interviewing with camera"), ``applauding" (confused with ``clapping"), ``riding mule" (confused with ``riding a horse"), ``tasting beer" (confused with ``drinking beer") or ``pretending to squeeze something". On the other hand, other classes like ``tearing something into two pieces", ``moving away from something with your camera", ``playing soccer", ``riding mountain bike", ``bartending" or ``hammer throw" seem to be sufficiently discriminating and unambiguous for both humans and machines to have high accuracy. 

We may also wonder if accuracy on shuffled videos is correlated in humans and machines, which would be useful to make the discovery of future temporal classes automatic. We test and find no significant correlation between the accuracy of humans on shuffled videos, and the accuracy of machines on shuffled videos. This suggests that a procedure to discover temporal classes without humans in the loop would require a more sophisticated methodology, and we hope that our labels can be help guide research in this direction. 

%\ls{describe statistical analysis}
%\lt{this analysis is a bit out of topic, as it has nothing to do with temporal relevancy. may need/want to tie it with the story.}
% \begin{figure}
% \centering
% \includegraphics[width=0.75\linewidth]{figures/human_vs_machine_r2plus1d_rgb.png}
% %\includegraphics[width=0.45\linewidth]{figures/human_vs_machine_r2plus1d_flow.png}
% \caption{{\bf Human Accuracy vs Machine Accuracy.} Visual complexity is correlated for humans and machines, harder classes for humans are also harder classes for machines.} %\lt{the plots need to be bigger, cant's see anything and the legends/labels are unreadable} \ls{maybe remove if short on space, and instead describe with words}}
% \label{fig:human_vs_machine_r3d}
% \end{figure}

==> human_vs_machine.tex <==
\paragraph{Humans vs. Machines}
% python notebook: plot acc and regression 
% python notebook: Plot Correlation by Group and Class (all datasets) 
%\lt{You may want to explain why you are presenting this analysis. It is introduced without context.}
Since our selection process is based on human perception, one may wonder if the recognition complexity of action classes similar for humans and machines. In other words, if a class is more ambiguous or harder for humans, is it also ambiguous or hard to identify for modern networks? We take the R(2+1)D model and measure correlation of per-class accuracy {\em without temporal shuffling} between humans and machines. %Results are shown in Fig.~\ref{fig:human_vs_machine_r3d}, 
We observe a positive correlation (Pearson correlation coefficient is 0.22) with high confidence (p-value is 0.001). Classes that are more ambiguous or harder for humans are also so for machines. For example both humans and machines find it hard to recognize  ``interviewing with camera" (confused with ``interviewing with camera"), ``applauding" (confused with ``clapping"), ``riding mule" (confused with ``riding a horse"), ``tasting beer" (confused with ``drinking beer") or ``pretending to squeeze something". On the other hand, other classes like ``tearing something into two pieces", ``moving away from something with your camera", ``playing soccer", ``riding mountain bike", ``bartending" or ``hammer throw" seem to be sufficiently discriminating and unambiguous for both humans and machines to have high accuracy. 

We may also wonder if accuracy on shuffled videos is correlated in humans and machines, which would be useful to make the discovery of future temporal classes automatic. We test and find no significant correlation between the accuracy of humans on shuffled videos, and the accuracy of machines on shuffled videos. This suggests that a procedure to discover temporal classes without humans in the loop would require a more sophisticated methodology, and we hope that our labels can be help guide research in this direction. 

%\ls{describe statistical analysis}
%\lt{this analysis is a bit out of topic, as it has nothing to do with temporal relevancy. may need/want to tie it with the story.}
% \begin{figure}
% \centering
% \includegraphics[width=0.75\linewidth]{figures/human_vs_machine_r2plus1d_rgb.png}
% %\includegraphics[width=0.45\linewidth]{figures/human_vs_machine_r2plus1d_flow.png}
% \caption{{\bf Human Accuracy vs Machine Accuracy.} Visual complexity is correlated for humans and machines, harder classes for humans are also harder classes for machines.} %\lt{the plots need to be bigger, cant's see anything and the legends/labels are unreadable} \ls{maybe remove if short on space, and instead describe with words}}
% \label{fig:human_vs_machine_r3d}
% \end{figure}

==> training_old.tex <==
\section{Effect of Training on the Temporal Dataset}

We have observed that the temporal categories exhibit different behavior when we use them as a test benchmark: on these classes, flow tends to be more powerful, and temporal shuffling affects accuracy more. We now address the question of whether temporal categories also exhibit different behaviour when used for training. The control sets we use are as described in Sec.~\ref{subsec:exp_details}.% a random set of classes of similar size to the temporal set. \lt{is this Union-179 or Union-722-small? need to be spelled out in text and all Tables.}

%In this section we study the impact of using the temporal categories to train video models. 
%Our hypothesis is that training networks with temporal convolutions on the temporal categories may lead to better temporal features. The reasoning behind this hypothesis is that if images are less informative, the network cannot use them to predict action labels, and thus will focus on the temporal information. 

\paragraph{Training on temporal categories vs training on all classes.} We compare the effect of training models on the union set of classes to training on the temporal categories (Temporal-173), and testing on the temporal classes. Our goal is to assess whether temporal features are better when they are trained on more diverse data, or when they are trained on the more specific set of temporal classes. To avoid differences in the number of videos, we use Union-722-small as control set. %\lt{are you sure it's not Union-179?}.
Our hypothesis is that training networks with temporal convolutions on the temporal categories may lead to better temporal features. To compare the two models fairly, we take the model initially trained on Union-722 and substitute the last fully-connected layer (of size 1024$\times$722) by one that maps to the temporal categories (of size 1024$\times$173). We then fine-tune this model on the temporal categories. The results in Table~\ref{tab:pretrained_motion_classes} confirm our hypothesis; training only on temporal classes seems beneficial, likely because the model can use the full capacity for fewer classes.

We may wonder if this behavior is specific to motion classes or generic to any subset of classes. 
We conduct a control experiment, applying the same procedure to fine-tune a model on the control set of randomly chosen classes Union-179. %\lt{???? this does not make sense, is the control Union-179 or Union-722-small? Correction is needed here or in the previous paragraph.}. %We keep the number of training videos the same for temporal and control classes for a fair comparison. 
%Our hypothesis is that training networks with temporal convolutions on the temporal categories may lead to better temporal features. %because when images are less informative, the network cannot ``cheat" and use image information to predict action labels, and thus will focus on the temporal information. 
We observe that the control set follows the same patter, and training on the specific set is beneficial as well. However, the gain in performance is much larger for the temporal categories. This suggests that even when the model is equipped with the ability to learn temporal information (such as in the case of R(2+1)D, which contains 3D convolutions), the network will not learn strong temporal features if optimized on non-temporal classes. Not surprisingly, R(2+1)D requires the appropriate training data (from temporal classes) to learn good temporal modeling. %\mdf{Also, a network pretrained on temporal features may find they are essentially noise for non-temporal concepts.  I.e. it may have to learn to ignore spurious correlations between certain kinds of visual features and motions.  If I understand figure 6 correctly though, this is not what happens?  I don't quite follow the dataset naming. } 
 
 

 

% \begin{table}
%     \centering
%     \begin{tabular}{l l l r r}
%         Input & Training & Test & Accuracy & Drop\\ \hline \hline
%         RGB & Union_{d} & Motion & 52.44\% & 9.77\%\\
%         Flow & Union_{d} & Motion & 45.18\% & 14.46\% \\
%         RGB & Motion & Motion & 58.12\% & \\
%         Flow & Motion & Motion & 52.82\% & \\ \hline
%         RGB & Union_{d} & Control & 63.56\% & 8.19\%\\
%         Flow & Union_{d} & Control & 58.10\% &5.00\% \\
%         RGB & Control & Control & 58.35\% \\
%         Flow & Control & Control & 55.19\%  \\ \hline
%     \end{tabular}
%     \vspace{.1cm}
%     \caption{{\bf Performance of R(2+1)D trained on the full set of classes vs trained on motion categories.}} %\lt{Are the control classes non-motion classes? Since at times we choose control classes from the full set and at other times we sample them from the  non-motion subset, I suggest to clarify in all tables by using Control-Full and Control-NM (non-motion)}
%     %\mdf{Is Union == $Motion \bigcup Control$?  So Union actually gives a better feature than Control when fine-tuned on Control?}
%     %\ls{this would probably look better as bar plot}\ls{need to make sure number of videos matches}\ls{run same experiment on ``static classes"}}
%     \label{tab:pretrained_motion_classes}
% \end{table}

\paragraph{Transfer learning across temporal categories.} In this experiment we examine the ability of a network trained on a subset of temporal categories (named ``seen") to recognize new temporal categories (named ``unseen"). Each of these two sets contain non-overlapping halves of the full set of temporal categories, and they are chosen randomly. More specifically, we train a network from scratch, on the ``seen" classes. We then freeze all weights (as in the experiment before) and fine-tune the final fully-connected layer on the ``unseen'' classes. This is equivalent to training a linear classifier on the `seen'' features. This tells us how well the knowledge of temporal classes transfers to new temporal classes. Our control set up is to train a model on a random set of categories from Union-722 of the same size as ``seen", referred to as the control set. Similarly, the last layer is fine-tuned on the ``unseen" temporal categories. If the random categories are just as useful to learn temporal categories, then the accuracy should be similar.
%We compare to a control set of categories, randomly selected from the full set of classes, to match the amount of classes in the ``seen" set. %\lt{We need to give the details of how the transfer learning is done. Are you training R(2+1)D from scratch on the seen classes? Do you then simply train a linear classifier on top of the last layer to recognize the unseen categories?} 
Table~\ref{tab:transfer} shows the results of this experiment. We observe that the transfer learning between the two subsets of temporal classes is more effective than that between the control subsets. This is an interesting fact, especially given that our analysis from Fig.~\ref{tab:test_motion_classes} suggested that recognition accuracy on temporal classes was overall lower than accuracy measured on the full dataset or the static classes. This suggests that the temporal classes share more common properties, which make the transfer learning more effective than across the control classes. One plausible conjecture is that this commonality is precisely the relevance of temporal information, which forces the network to learn general temporal features that transfer well across temporal classes.

\begin{table}
    \centering
    \begin{tabular}{l l l r }
        Input & {Training Set} & {Test Set} & Accuracy  \\ \hline \hline
        RGB & Seen Temporal & Unseen Temporal & 44.64\%\\
        Flow & Seen Temporal & Unseen Temporal & 45.43\% \\
        RGB & Seen Control & Unseen Temporal & 41.50\% \\
        Flow & Seen Control & Unseen Temporal & 41.95\% \\ \hline
    \end{tabular}
    \vspace{.1cm}
    \caption{{\bf Transfer learning within temporal categories using R(2+1)D.}}
    \label{tab:transfer}
\end{table}

\paragraph{Learning from temporal categories leads to more temporally-aware models. } In this experiment we measure how much temporal structure is learned by the R(2+1)D network trained on temporal categories as opposed to regular categories. We train two models, one on the temporal categories and one on Union-179. We train on the original videos, but test after randomly shuffling the frames. The model trained and tested on randomly selected classes serves as control in this experiment. Table~\ref{tab:shuffling_at_train} shows the results, where drop refers to the difference in accuracy. The drop is calculated relative to the accuracy. Previous work has shown that shuffling~\cite{Huang2018WhatMA, gcpr18} does not affect performance greatly even for networks with temporal convolutions. Our experiment suggests that this drop in performance is much larger for the temporal categories. This makes sense as they require temporal information for discrimination. 

\begin{table}
    \centering
    \begin{tabular}{l l r r}
        Input &  {Train/Test} & {Drop Video} & {Drop Clip}\\ \hline \hline
        RGB & Temporal & $\nabla$ 23.31\% & $\nabla$ 15.96\% \\
        Flow & Temporal & $\nabla$ 54.78\% & $\nabla$ 42.06\% \\  \hline 
        RGB & Union-179  & $\nabla$ 16.96\%& $\nabla$ 6.98\% \\
        Flow & Union-179  & $\nabla$ 48.82\% & $\nabla$ 24.73\% \\ \hline
        % %R(2+1)D (RGB + Flow) & ??\% & ??\% & ??\%  \\
        % R2D (RGB) & 24.39\% & 35.21\% & 31.83\%  \\  
        % R2D (Flow) & 25.87\% & 22.92\% & 22.23\%  \\
    \end{tabular}
    \vspace{.1cm}
    \caption{{\bf Effect of shuffling on models trained on temporal categories and on models trained on random classes.} }%\vg{Not clear what the Drop \% are comparing against. Also maybe replace' with 'Drop Video level accuracy' and Drop in Clip level accuracy' }} }
    \label{tab:shuffling_at_train}
    \vspace{-0.3cm}
\end{table}


% \begin{table*}
%     \centering
%     \begin{tabular}{l l r r r r r}
%         Architecture &  Training/testing & Accuracy & \specialcell{Accuracy\\Video Shuffle} & \specialcell{Drop\\Video Shuffle} &\specialcell{Accuracy\\Clip Shuffle} & \specialcell{Drop\\Clip Shuffle}\\ \hline \hline
%         R(2+1)D (RGB) & Motion classes & 58.12\% & 44.57\% & $\nabla$ 23.31\% & 48.84\% & $\nabla$ 15.96\% \\
%         R(2+1)D (Flow) & Motion classes & 52.82\% & 23.88\% & $\nabla$ 54.78\% & 30.60\% & $\nabla$ 42.06\% \\  \hline 
%         R(2+1)D (RGB) & Control classes & 63.56\% & 52.78\% & $\nabla$ 16.96\% & 59.12\% & $\nabla$ 6.98\% \\
%         R(2+1)D (Flow) & Control classes & 58.10\% & 33.22\% & $\nabla$ 48.82\% & 43.73\% & $\nabla$ 24.73\% \\ \hline
%         % %R(2+1)D (RGB + Flow) & ??\% & ??\% & ??\%  \\
%         % R2D (RGB) & 24.39\% & 35.21\% & 31.83\%  \\  
%         % R2D (Flow) & 25.87\% & 22.92\% & 22.23\%  \\
%     \end{tabular}
%     \vspace{.1cm}
%     \caption{{\bf Effect of shuffling on models trained on motion categories and on models trained on random classes } }
%     \label{tab:shuffling_at_train}
% \end{table*}


% \ls{yet another baseline would be to keep a task fixed and train with motion classes vs. on random classes }
% Here I would like to do another experiment with shuffling. In the previous shuffling experiment, we both train and test on different data. It is not clear if the drop comes from the task we're testing or from training on motion data. Here, we keep the task fixed (eg. unseen random classes) and train on seen motion classes vs. seen random classes. Now I'll shuffle at test time, and we should see a larger drop in the model that was trained using the motion categories. I'll put the results in Table~\ref{tab:shuffling_at_train}. 

% \begin{table*}
%     \centering
%     \begin{tabular}{l l r r r r r}
%         Architecture &  Training & Accuracy & \specialcell{Accuracy\\Video Shuffle} & \specialcell{Drop\\Video Shuffle} &\specialcell{Accuracy\\Clip Shuffle} & \specialcell{Drop\\Clip Shuffle}\\ \hline \hline
%         R(2+1)D (RGB) & Motion & --\% & --\% & $\nabla$ --\% & --\% & $\nabla$ --\% \\
%         R(2+1)D (Flow) & Motion & --\% & --\% & $\nabla$ --\% &--\% & $\nabla$ --\% \\  \hline \hline
%         R(2+1)D (RGB) & Control & --\% & --\% & $\nabla$ --\% & --\% & $\nabla$ --\% \\
%         R(2+1)D (Flow) & Control & --\% & --\% & $\nabla$ --\% & --\% & $\nabla$ --\% \\
%         % %R(2+1)D (RGB + Flow) & ??\% & ??\% & ??\%  \\
%         % R2D (RGB) & 24.39\% & 35.21\% & 31.83\%  \\  
%         % R2D (Flow) & 25.87\% & 22.92\% & 22.23\%  \\
%     \end{tabular}
%     \vspace{.1cm}
%     \caption{{\bf Shuffling} }
%     \label{tab:shuffling_at_train}
% \end{table*}

% \paragraph{Experiment 4: }{\em Training on motion categories leads to more discriminative filter responses.} In this experiment we measure the standard deviation (std) of temporal filter responses at conv1 layer of R(2+1)D models trained on motion categories and random categories over every 5 epoch from 10 to 75 epochs. Fig.~\ref{fig:std_motion_vs_random} shows that the std reduces as the number of epochs increases, i.e. as the filters become more discriminative; and the std obtained from models trained on motion categories are consistently lower that trained on random categories.

% \begin{figure}
% % \centering
% \includegraphics[width=\linewidth]{figures/std_motion_vs_random.png}
% \caption{{\bf Average standard deviation of temporal filter responses at conv1 layer of R(2+1)D models trained on motion categories and random categories.} \szha{ TODO: swap figure with correct model}} 
% \label{fig:std_motion_vs_random}
% \end{figure}






